Matrix Norms in Data Streams: Faster, Multi-Pass and Row-Order

A central problem in data streams is to characterize which functions of an underlying frequency vector can be approximated efficiently. Recently there has been considerable effort in extending this problem to that of estimating functions of a matrix that is presented as a data-stream. This setting generalizes classical problems to the analogous ones for matrices. For example, instead of estimating frequent-item counts, we now wish to estimate "frequent-direction" counts. A related example is to estimate norms, which now correspond to estimating a vector norm on the singular values of the matrix. Despite recent efforts, the current understanding for such matrix problems is considerably weaker than that for vector problems. We study a number of aspects of estimating matrix norms in a stream that have not previously been considered: (1) multi-pass algorithms, (2) algorithms that see the underlying matrix one row at a time, and (3) time-efficient algorithms. Our multi-pass and row-order algorithms use less memory than what is provably required in the single-pass and entrywise-update models, and thus give separations between these models (in terms of memory). Moreover, all of our algorithms are considerably faster than previous ones. We also prove a number of lower bounds, and obtain for instance, a near-complete characterization of the memory required of row-order algorithms for estimating Schatten $p$-norms of sparse matrices.

==> sec_eigen_values.tex <==
\section{Top Singular Values}
\label{sec:top single values}
The results of \cite{andoni2013eigenvalues} approximate 
the top eigen/singular values of a matrix using a bilinear sketch given by Gaussian matrices
(note that if the input matrix is symmetric, then the signs of the eigenvalues can also be preserved).
This section shows that similar guarantees can be achieved 
using a generic OSE  instead of Gaussian matrix.
By using a sparse OSE matrix,
we obtain better update time than \cite{andoni2013eigenvalues}. 

\begin{theorem}
\label{thm:l1 heavy hitters}
Fix $\epsilon>0$ and integers $n, k\ge1$. Let $A\in \bbR^{n\times n}$ be a 
symmetric matrix and let $\lambda_{i}^*(A)$ be the $i$-th largest eigenvalue of 
$A$ in absolute value.
Then there is a linear sketch of $A$, using space $O(\epsilon^{-2}k \log n)^2$, from which one can produce values $\tilde{\lambda}_1, \tilde{\lambda}_2,\ldots, \tilde{\lambda}_k$, 
such that% there exists a permutation $\rho:[k]\rightarrow [k]$, and
\[
\Pr\left[\forall i\in [k]:|\tilde{\lambda}_{i}(A)-{\lambda_i^*}(A)|\le \epsilon|{\lambda}^*_i(A)| + \frac{1}{k}\sum_{i>k} |{\lambda}^*_i(A)|\right]\ge 5/9.
\]
% Then there is a linear sketch of $A$, using space $O(\epsilon^{-2}k \log n)^2$, from which one can produce a set of values $S=S_1\cup S_2\subset \bbR$ with $|S| =O(\epsilon^{-2}k \log n)$ and $|S_1|=k$,
%$\tilde{\lambda}_1, \tilde{\lambda}_2,\ldots, \tilde{\lambda}_k$, 
%such that with probability at least $5/9$
% there exists a permutation $\rho:[k]\rightarrow [k]$, and
%\begin{enumerate}
%\item $\forall i\in [k], \exists \tilde{\lambda}_i\in S_1: |\tilde{\lambda}_{i}-{\lambda_i^*}(A)|\le %%\epsilon|{\lambda}^*_i(A)| + \frac{1}{k}\sum_{i>k} |{\lambda}^*_i(A)|$;
%\item  $\forall s\in S_2: |s|\le \frac{1}{k}\sum_{i>k} |{\lambda}^*_i(A)|$.
%\end{enumerate}
For each update to the matrix $A$, the skech can be updated in time $O(\log^2 n/\epsilon^2)$.
\end{theorem}
%\rnote{I have several problems here.
%(1) This deviates from our prelims,
%which says that $\lambda_i(A)$ are order in decreasing value,
%and $\tilde\lambda_i(A)$ are in decreasing absolute value.
%We should write it consistently with the rest of our paper.
%(2) I think the statement is too strong, 
%because the order between positive and negative eigenvalues might change.
%For example, if $\lambda_k(A) \approx -\lambda_{k+1}(A)$ (almost equal), 
%then the estimator for $\lambda_k$ is not likely to get the correct sign.
%The same issue arises in lemma 5.2...
%(3) How does thm 5.1 follow from lemma 5.2? 
%(I see AN13 say it is by setting $\phi=\Theta(1/k)$, 
%but they give no more details and the problem is the same.)
%Our lemma 5.2 has two types of additive error,
%one is $\eps^2\phi \text{tail} < \phi \text{tail}$ and is thus fine,
%the second is $\lambda_{1/\phi}$ (we're missing plus 1) which can be large, no?
%}
%\lynote{The statement of the theorem should be fine. 
%(1) It looks like not possible to write $\lambda_i$ ordered by the original orders,
%since this theorem can only compare their absolute values.
%In order to streamline, I made $\lambda^*$.
%(2) The statement of the theorem does not relates to the
%order the eigenvalues. It says that for any $\lambda_i^*(A)$
%there exists an eigenvalue of the sketch that corresponds
%to it.
%(3) I added the following proof.}
\begin{proof}
The proof of this theorem follows from Lemma~\ref{lemma:top eigenvalues}
by setting $\phi=1/(ck)$ for some constant $c\ge2$. Indeed it follows that 
$\epsilon^2 \phi \sum_{i=1/\phi + 1}|{\lambda^*}_i(A)| 
\le \frac{1}{k}\sum_{i=k + 1}|{\lambda^*}_i(A)|$
and $|{\lambda^*}_{1/\phi}|(A) \le \frac{1}{(c-1)k} \sum_{i= k +1}^n|{\lambda^*}_i(A)|$.
The proof of Lemma~\ref{lemma:top eigenvalues} is very similar to the proof of Lemma 3.4 
of \cite{andoni2013eigenvalues}, except that we give a more fine-grained 
statement regarding the mapping between the eigenvalues. 
Their sketch is of the form $GAG^T$, 
where $G$ is a column-normalized Gaussian matrix. 
Our sketch is similar, except that $G$ is an OSE matrix, 
specifically it is both $(\epsilon, 1/\poly n, \phi^{-1})$-OSE
and $(0.1, 1/\poly n, \phi^{-1}\eps^{-2})$-OSE. 
The existence of such $G$ follows from Theorem \ref{thm:cohen sparse ose},
and its sparsity determines our update time.
\end{proof}



\begin{theorem}
Fix $\epsilon>0$ and integers $1\le m\le n, k\ge1$. Let $A\in \bbR^{n\times m}$ be a real 
 matrix. Then there is a linear sketch of $A$, using space $O[(k\epsilon^{-2} \log n)^2]$, 
from which one can produce values $\hat{\sigma}_i$ for $i\in [k]$, satisfying the following with at
least $5/9$ sucess probability,
\[
|\sigma_{i}^2(A)-\hat{\sigma}^2_i|\le \epsilon \sigma_i^2(A) + \frac{1}{k}\sum_{i>k} \sigma_i^2(A).
\]
%from which one can  produce a set of values $S=S_1\cup S_2\subset \bbR$ with $|S| =O(\epsilon^{-2}k \log n)$ and $|S_1|=k$,
%$\tilde{\lambda}_1, \tilde{\lambda}_2,\ldots, \tilde{\lambda}_k$, 
%such that with probability at least $5/9$
% there exists a permutation $\rho:[k]\rightarrow [k]$, and
%\begin{enumerate}
%\item $\forall i\in [k], \exists \tilde{\sigma}_i\in S_1: |\tilde{\sigma}^2_{i}-{\sigma_i^2}(A)|\le \epsilon|{\sigma}^2_i(A)| + \frac{1}{k}\sum_{i>k} |\sigma^2_i(A)|$;
%\item  $\forall s\in S_2: s^2\le \frac{1}{k}\sum_{i>k} {\sigma}_i^2(A)$.
%\end{enumerate}
%produce a set of values $S\subset \bbR$ 
%with $|S| =O(\epsilon^{-2}k \log n)$
%one can produce values $\hat{\sigma}_i$ for $i\in [k]$, satisfying the following with at
%least $5/9$ sucess probability,
%\[
%\Pr\left[\forall i\in [k], \exists \tilde{\sigma}_i\in S: |\sigma_{i}^2(A)-\hat{\sigma}^2_i|\le \epsilon \sigma_i^2(A) + \frac{1}{k}\sum_{i>k} \sigma_i^2(A)\right]\ge 5/9.
%\]
%\[
%|\sigma_{i}^2(A)-\hat{\sigma}^2_i|\le \epsilon \sigma_i^2(A) + \frac{1}{k}\sum_{i>k} \sigma_i^2(A).
%\]
For each update to the matrix $A$, the sketch can be updated in time $O(\log^2 n/\epsilon^2)$.
\end{theorem}
This theorem follows from the Lemma~\ref{lemma:singular value heavy hitters} (by setting $\phi=O(1/k)$, with 
an identical argument as used in the proof of Theorem~\ref{thm:l1 heavy hitters}), 
which is a modification of \cite[Lemma 3.5]{andoni2013eigenvalues}. 
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> sec_general_norm.tex <==
\section{Unitarily Invariant Matrix Norms}\label{sec: unitarily invariant}

In this section we show how to use a generic OSE to approximate any unitarily invariant matrix norm $l(A)$ using the sketch $GAH^T$ for OSE matrices $G,H\in\R^{t\times n}$ and $t=(\idim(A)/\epsilon)^{O(1)}$. 
As we show in Appendix~\ref{sec:proofs of sec ui}, it is necessary that $t=(\sr(A)/\epsilon)^{\Omega(1)}$,
where $\sr(A) \coloneqq (\sum_{j\geq1}\sigma_j^2)/\sigma_1^2\leq\idim(A)$ is the \emph{stable rank} of $A$.
It is an open problem to determine whether a smaller sketch with $t = \sr(A)^{O(1)}$ suffices for approximating $l(A)$.
Theorem~\ref{thm:norm non-psd Q-norm} can be used to make some progress on the problem by showing that $t=\sr(A)^{O(1)}$ dimensions suffices for a class of norms called $Q$-norms. 
OSEs embedding into $t=O(\sr(A))$ are known to suffice for approximate matrix multiplication algorithms~\cite{cohen2015optimal}.

Since we approximate $l(A)$ using a linear sketch, we immediately have a one-pass streaming algorithm.
Furthermore, the sketch is bilinear and universal, i.e., it does not depend on the norm $l$ except through the dimension of the sketch.
Our main technical results describe the accuracy of the bilinear sketch for approximating functions of the input matrix.  
They are Theorem~\ref{thm:norm psd} for PSD matrices and Theorem~\ref{thm:norm non-psd Q-norm} for general matrices and $Q$-norms, which is postponed Appendix~\ref{app:qnorm}. 
Their accuracy guarantees actually depend on the input's singular values,
and thus their effectiveness depends on the norm at hand
and/or on the intrinsic dimension (or stable rank) of the input.
%%%%%We also provide a lower bound in Appendix~\ref{sec: intdim lower bounds} that shows the space complexity of approximating these functions depends polynomially on the stable rank.

Throughout, let $I_d$ denote the identity matrix of order $d$.
By convention, we extend a norm $l$ on $n\times n$ matrices to 
smaller-order square matrices as follows.
For a matrix $A\in\R^{d\times d}$ with $d<n$, we let 
$
  A' \eqdef \left( \begin{smallmatrix}
          A & 0 \\ 0 & 0
       \end{smallmatrix} \right)
  % \left(\begin{array}{cc} A & 0 \\ 0 & 0\end{array}\right)
       \in\R^{n\times n}
$
and define $l(A)\eqdef l(A')$.

\begin{theorem}
\label{thm:norm psd}
Let $G\in\bbR^{t\times n}$ be an $(\epsilon, \delta, O(d\log n))$-OSE matrix
for integers $1\le d\le t\le n$
and some $\eps\in(1/n^9,1/2)$ and $\delta\in(0,1/2)$.
Then for every PSD matrix $A\in \bbR^{n\times n}$,
and every unitarily invariant norm $l(\cdot)$ on ${n\times n}$ matrices,
with probability at least $1-2\delta n$, 
\begin{equation}
  (1-\epsilon) l(A)
  \le l(GAG^T)
  \le (1+O(\epsilon))
l(A)%l(\diag(\lambda_1, \ldots, \lambda_d))
        +   O\left( \frac{l(I_{d})}{d}\sum_{i=d+1}^n \lambda_i
  \right) .\label{eq: psd norms theorem}
\end{equation}
%\begin{equation}
%  (1-O(\epsilon))\ l(A)
%  \le l(GAG^T)
%  \le (1+O(\epsilon))
%  \left( l(\diag(\lambda_1, \ldots, \lambda_d))
%        + \frac{l(I_d)}{d}\sum_{i=d+1}^n \lambda_i
%  \right) .\label{eq: psd norms theorem}
%\end{equation}
where $\lambda_1\geq \ldots\geq \lambda_n\ge0$ are the eigenvalues of $A$.
\end{theorem}
%\lynote{For RHS, the first term of $l(\lambda_1, \lambda_2, \ldots, \lambda_d)$ is
%changed to $l(A)$. For the second term, we changed the numerator to $O(I_{d})$ and
%OSE is changed to dimension $d\log n$.}
%\rnote{In the LHS, I removed the big O since the proof gives it.
%I've also pushed these small changes to the examples below.}

We continue with applications of the theorem, 
before proving it in Section~\ref{sec:proof of psd theorem}.
%
%\subsubsection{Examples}
%A key feature of this theorem is that $l(A)$ can be estimated using the matrix $GAG^T\in\R^{t\times t}$, which is a linear sketch of $A$, and moreover does not depend on $l$.
%(Of course, using the sketch to produce an actual estimate does depend on $l(\cdot)$.) 

\paragraph{Low intrinsic dimension.}
%
The bound in \eqref{eq: psd norms theorem} is particularly useful 
when the eigenvalues of $A$ are decaying.
%
Suppose we have an upper bound on the intrinsic dimension of $A$,
namely, $\idim(A)\le r$.
Then we can bound $\sum_{i\ge1} \lambda_i \le r \lambda_1$,
and by \eqref{eq: psd norms theorem} we have that 
\begin{equation} \label{eq:low_idim}
  (1-\epsilon) l(A)
  \le l(GAG^T)
  \le (1+O(\epsilon))
       l(A) + O\left(\frac{l(I_{d})}{d} r \lambda_1 
      \right) .
\end{equation}
As a first example, if $l(\cdot)$ is the Schatten $p$-norm for $p>1$,
we can choose $d=(r/\eps)^{1+1/(p-1)}$,
which determines $t^2$, the dimension of the sketch.
We get that 
$
  (\normSp{I_d}/d) \cdot r \lambda_1
  = d^{1/p-1} r \lambda_1
%  = (r/\eps)^{\frac{p}{p-1}\cdot \frac{1-p}{p}}\cdot r \lambda_1
  \le \eps \normSp{A}
$,
and now \eqref{eq:low_idim} implies that
$
%  (1-O(\epsilon)) \normSp{A}
  \normSp{GAG^T}
  \in (1\pm O(\epsilon))\ \normSp{A} .
$

A second example is the following straightforward extension.
Fix $\alpha>0$ and let $l$ be a norm such that 
%\[
  for all $d\leq n$, 
  $l(I_d) \leq d^{1-\alpha} l(I_1)$.
%\]
We can choose $d=(r/\eps)^{1/\alpha}$,
which determines $t^2$, the dimension of the sketch.
We get that 
$
  (l(I_d)/d) \cdot r \lambda_1
  \le d^{-\alpha} l(I_1) \cdot r \lambda_1
  \le \eps\ l(A)
$,
and now \eqref{eq:low_idim} implies that
$
  l(GAG^T)
  \in (1\pm O(\eps))\ l(A) .
$

A third example is where $l(\cdot)$ is the Ky Fan $k$-norm,
defined as $\normKF{A}=\sigma_1+\ldots+\sigma_k$ where 
$\sigma_1\ge\sigma_2\ge...$ are the singular values of $A$.
In our case where $A$ is PSD, $\normKF{A} = \lambda_1+\ldots+\lambda_k$.
%
By choosing $d=kr/\eps$,
which determines $t^2$, the dimension of the sketch,
we get 
$
  (\normKF{A}/d)\cdot r \lambda_1
  \leq (kr/d) \lambda_1
  \leq \eps \normKF{A}
$,
and now \eqref{eq:low_idim} implies that
%  (1-O(\epsilon)) \normKF{A}
$
  \normKF{GAG^T}
  \in (1\pm O(\epsilon))\ \normKF{A} .
$

Notice that all these examples use the same sketch,
and more generally, a single sketch can be used to estimate many norms.
In fact, with high probability the sketching succeeds 
--- this is an event that does not depend on the desired norm ---
in which case the accuracy bounds \eqref{eq: psd norms theorem}
hold simultaneously for \emph{all the relevant norms}.
We note that this statement actually follows from our proof,
although we do not formalize it for sake of brevity.

\begin{proposition}
\label{prop:alg psd}
Fix $\alpha>0$ and let $\calL_\alpha$ be the set of all unitarily invariant 
norms $l$ on $\R^{n\times n}$ 
such that $l(I_d) \leq d^{1-\alpha} l(I_1)$ for all $d\leq n$.
There exists a randomized one-pass streaming algorithm $\calA$ 
that takes as input any PSD matrix $A\in \bbR^{n\times n}$ with $\idim(A)\le r$,
and outputs a square matrix $D$ of order $O(r/\epsilon)^{1/\alpha}$,
such that for every $l\in\calL_\alpha$, 
%there exits a function $f$, which can be computed in $\poly(r/\epsilon)$ time, such that
\[
  \Pr\Big[ l(D) \in (1\pm \epsilon)\ l(A) \Big] \ge 9/10 .
\]
Moreover, $\calA$ uses $\poly(r\log(n)/\epsilon)$ bits of space 
and has update time $O(\epsilon^{-2}\log^2 n)$.
\end{proposition}

\begin{proof}
Algorithm $\calA$ follows Theorem~\ref{thm:norm psd}
and maintains the linear sketch $D=GAG^T$.
Its accuracy follows from the second example above, 
and it remains to bound the algorithm's space and update time.
If the OSE matrix $G$ is constructed using Theorem~\ref{thm:cohen sparse ose},
then every column of $G$ has $O(\epsilon^{-1}\log n)$ non-zero entries,
and an update to $D$ (given an update to one entry of $A$) 
can be implemented in time $O(\epsilon^{-2}\log^2 n)$
The space used by the algorithm is only for storing the sketch matrix $GAG^T$,
which has size $O(d^2) = O(r/\eps)^{2/\alpha}$ words.  
\end{proof}

\subsection{Proof of Theorem~\ref{thm:norm psd}}
\label{sec:proof of psd theorem}

Before the proof we need three technical lemmas. 
Lemma~\ref{lemma:ose preserves eigenvalues} extends \cite[Lemma 3.2]{andoni2013eigenvalues}  from (multiplying the input matrix by) Gaussian matrices to general OSEs.
It asserts that the nonzero eigenvalues of $SAS^T$ approximate that of $A$, including the sign.
The proof of Theorem~\ref{thm:norm psd} is based on 
applying Lemma \ref{lemma:ose preserves eigenvalues}, 
separately for each ``block'' of eigenvalues 
(though $A$ is not required to be block-diagonal).

\newcommand{\osepreserveseigenvalueslemma}{Let $S\in\R^{t\times n}$ be an $(\epsilon, \delta, d)$-OSE and let $A\in\R^{n\times n}$ be a symmetric matrix of rank $r\leq d$.
Then with probability at least $1-\delta$, 
we have $\rank(SAS^T)=r$ and there exists a permutation $\rho:[r]\to[r]$ such that
\[
  \forall i\in[r], \qquad
  \tilde{\lambda}_i(SAS^T) \in (1\pm 3\eps) \tilde{\lambda}_{\rho(i)}(A) ,
%\left|\tilde{\lambda}_i(SAS^T)-\tilde{\lambda}_i(A)\right|\le 3\epsilon|\tilde{\lambda}_i(A)|,\text{ for }i=1,2,\ldots,\rank(A),
\]
where $\tilde{\lambda}_i(M)$ is the $i$th non-zero eigenvalue of $M$ in decreasing order.
}
\begin{lemma}
\label{lemma:ose preserves eigenvalues}
\osepreserveseigenvalueslemma
\end{lemma}

\newcommand{\upperboundallnormslemmatext}{Let $l(\cdot)$ be a unitarily invariant norm on matrices in $\R^{n\times n}$,
and let $S\in\R^{t\times n}$ be an $(\epsilon, d\delta/n, d)$-OSE matrix.
Then for every symmetric matrix $A\in\R^{n\times n}$, 
with probability at least $1-\delta$,
\[
%  l(SAS^T)
 % \le (1+O(\epsilon)) \frac{n l(I_d)}{d}\|A\|_{S_\infty},
  l(SAS^T)
  \le (1+O(\epsilon))\ \ceil{n/d}\ l(I_d)\ \norm{A}_{S_\infty}, 
\]
where $I_d$ is the identity matrix of order $d$.
}
\begin{lemma}
\upperboundallnormslemmatext
\label{lemma:upper bound norm for all norm}
\end{lemma}

\newcommand{\variationalcharpropositiontext}{
  If $l(\cdot)$ is a symmetric norm on $\R^m$ and $l(A) := l(\lambda_1(A), \lambda_2(A), \ldots, \lambda_m(A))$, then
  \begin{align*}
    l(A) = \max &\;\; l((|u_1^T A v_1|, |u_2^T A v_2|, \ldots, |u_m^TAv_m|)^T)\\
    s.t.\;\; & u_1,\ldots,u_m\in\calS^{m-1}\text{ are orthogonal}\\
    & v_1,\ldots,v_m\in\calS^{n-1}\text{ are orthogonal}.
  \end{align*}
}
\begin{proposition}\label{prop: variational characterization of norm}
\variationalcharpropositiontext
\end{proposition}
%We are now prepared to prove Theorem~\ref{thm:norm psd}.
\begin{proof}[Proof of Theorem~\ref{thm:norm psd}]
We first show the second inequality in \eqref{eq: psd norms theorem}. 
By the Spectral Theorem, $A=U\Lambda U^T$, 
where $U\in\R^{n\times n}$ is orthonormal 
and $\Lambda=\diag(\lambda_1, \ldots, \lambda_n)$.
By Lemma~\ref{lemma:ortho trans ose}, 
also $G'=GU$ is an $(\epsilon, \delta, O(d\log n))$-OSE matrix, 
and we only need to consider the case where $A=\Lambda$ is a diagonal matrix.
%
We group the eigenvalues into buckets. 
Let $\Lambda_0$ be the top $d$ eigenvalues. 
For the rest, %set $\alpha =2$, and 
for $k=1,2,\ldots$ define 
$\Lambda_k = \{\lambda_j: j>d \text{ and } \lambda_1/2^{k}< \lambda_j\le \lambda_1/2^{k-1} \}$.
%$O(\eps^{-1}\log n)$.
Since the norm is monotonic in the eigenvalues of $A$, we can ignore eigenvalues smaller than $\epsilon\lambda_1/n$, i.e., treat them as zero.
Indeed, by the triangle inequality, zeroing them can decrease $l(A)$ 
by at most $\eps \lambda_1 l( I_1) \le \eps\ell(A)$.
Thus, the effective number of buckets is $b = O(\log (n/\eps)) = O(\log n)$.
For each $k\ge1$, if bucket $\Lambda_k$ is small, namely, $|\Lambda_k|\le d$, 
then we add this bucket to $\Lambda_0$ (so now bucket $\Lambda_k$ is empty).
For simplicity, we use the same notation $\Lambda_k$ for the new buckets
(although formally this step defines a new set of buckets $\Lambda'_k$).
% $\Lambda_0:=\cup_{i\ge 0: |\Lambda_i|\le d} \Lambda_i$ 
With the new buckets, $|\Lambda_0| \le (b+1)d = O(d\log n)$,
and for every $k\ge 1$, either $|\Lambda_k|=0$ or $|\Lambda_k|\ge d$.

With slight abuse of notation, 
we denote by $\Lambda_k$ also the corresponding diagonal matrix, which is 
obtained from $\Lambda$ by zeroing out the eigenvalues not in $\Lambda_k$. 
Thus $\Lambda = \sum_{k\ge 0}\Lambda_k$,
and by the triangle inequality, 
\[
  l(G\Lambda G^T)
  = l\Big( \sum_{k\ge 0} G \Lambda_k G^T \Big)
  \le l(G\Lambda_0 G^T)+ \sum_{k\ge1} l(G\Lambda_i G^T).
\]
By Lemma \ref{lemma:ose preserves eigenvalues}, 
with probability $1-\delta$ we have 
$ l(G\Lambda_0 G^T)\le (1+O(\epsilon))\ l(\Lambda_0)\le (1+O(\epsilon))l(A)$.
Let this event be denoted $E_0$.

Now we apply Lemma \ref{lemma:upper bound norm for all norm} 
to each non-empty block $k=1,\ldots,b$. 
Specifically, in block $k$ we apply the lemma treating $l$ as a norm with dimension $|\Lambda_k|$.
Thus, for each such $k$,
with probability at least $1-\delta \card{\Lambda_k}/d$, we have that
$l(G\Lambda_k G^T)
  \leq (1+O(\epsilon)) \frac{|\Lambda_k|}{d} l(I_d)\|\Lambda_k\|$. 
By a union bound over the $b$ blocks, with probability at least 
$1-\delta \frac{1}{d}\sum_{k\geq1}|\Lambda_k|\geq 1-\delta (n-d)/d$, 
we have
\[
 \sum_{k\ge1} l(G\Lambda_k G^T)
 \le (1+O(\epsilon)) \frac{l(I_d)}{d} 
     \sum_{k\ge1} \card{\Lambda_k}\cdot \norm{\Lambda_k}_2 
 \le O(1) \frac{ l(I_d)}{d} \sum_{i=d+1}^n\lambda_i. %\|A\|_{S1},
\]
Let this event be denoted by $E_1$. 
This completes the upper bound in \eqref{eq: psd norms theorem}.

Next, we show the lower bound on $\ell(GAG^T)$.
%we use that $\|G\Lambda G^T\|_{Sp}\ge \lambda_{t}(G G^T)\|\Lambda\|_{Sp}$.
The PSD matrices $GAG^T$ and $\sqrt{\Lambda}G^TG\sqrt{\Lambda}$ 
have the same set of non-zero eigenvalues, 
hence $\ell(GAG^T) = \ell(\sqrt{\Lambda}G^TG\sqrt{\Lambda})$.
By the variational characterization of $\ell(\cdot)$,
as given in Proposition~\ref{prop: variational characterization of norm},
\[
  \ell(\sqrt{\Lambda}GG^T\sqrt{\Lambda})
  \ge \ell(\diag(e_1^T\sqrt{\Lambda}G^TG\sqrt{\Lambda}e_1, 
      \ldots, 
      e_n^T\sqrt{\Lambda}G^TG\sqrt{\Lambda}e_n)).
\] 
For each $i\in [n]$, since $G$ is an OSE matrix (for dimension at least $1$),
with probability at least $1-\delta$ we have
$e_i^T\sqrt{\Lambda}G^TG\sqrt{\Lambda}e_i = \lambda_i \langle Ge_i, Ge_i\rangle
\ge (1-\epsilon)\lambda_i$. 
By a union bound, with probability at least $1-n\delta$ we have
$\ell(GAG^T)\ge (1-\epsilon) \ell(A)$, which event we denote by $E_2$. 

Combining the two inequalities we find with probability at least 
$1-\Pr(\bar E_0)-\Pr(\bar E_1)-\Pr(\bar E_2) \geq 1-2n\delta$ 
both inequalities in~\eqref{eq: psd norms theorem} hold.  
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> sparse_variance.tex <==
% a tikz graph 
\begin{center}
\begin{tikzpicture}
\node at (-5,1) (nodei1) {$i_1$};
\node at (-3,1) (nodej1) {$j_1$};
\node at (-1,1) (nodei2) {$i_2$};
\node at (1,1) (nodej2) {$j_2$};
\node at (3,1) (nodei3) {$i_3$};
\node at (5,1) (nodej3) {$j_3$};
\node at (-5,-1) (nodei1p) {$i_1'$};
\node at (-3,-1) (nodej1p) {$j_1'$};
\node at (-1,-1) (nodei2p) {$i_2'$};
\node at (1,-1) (nodej2p) {$j_2'$};
\node at (3,-1) (nodei3p) {$i_3'$};
\node at (5,-1) (nodej3p) {$j_3'$};
\draw [dashed] (nodej1) -- (nodei2) node[midway, above] {$a_{j_1, i_2}$};
\draw [dashed] (nodej2) -- (nodei3) node[midway, above] {$a_{j_2, i_3}$};
\draw [dashed, out=15, in=165] (nodei1) to node[midway, above, sloped] {$a_{j_3, i_1}$} (nodej3) ;
\draw [dashed] (nodej1p) -- (nodei2p) node[midway, below] {$a_{j_1', i_2'}$};
\draw [dashed] (nodej2p) -- (nodei3p) node[midway, below] {$a_{j_2', i_3'}'$};
\draw [dashed, out=-20, in=-160] (nodei1p) to node[midway, below, sloped] {$a_{j_3', i_1'}$} (nodej3p) ;
\draw (nodei1) -- (nodej1);
\draw (nodei1p) -- (nodej1p);
\draw (nodei2) -- (nodej2p);
\draw (nodei2p) -- (nodej2);
\draw (nodei3) -- (nodei3p);
\draw (nodej3) -- (nodej3p);
\end{tikzpicture}
\end{center}
